The Next White (NEW) detector

Conceived to host 5 kg of xenon at a pressure of 15 bar in the fiducial volume, the NEXT- White (NEW) apparatus is currently the largest high pressure xenon gas TPC using electroluminescent amplification in the world. It is also a 1:2 scale model of the NEXT-100 detector scheduled to start searching for $\beta\beta 0\nu$ decays in 136Xe in 2019. Both detectors measure the energy of the event using a plane of photomultipliers located behind a transparent cathode. They can also reconstruct the trajectories of charged tracks in the dense gas of the TPC with the help of a plane of silicon photomultipliers located behind the anode. A sophisticated gas system, common to both detectors, allows the high gas purity needed to guarantee a long electron lifetime. NEXT-White has been operating since October 2017 at the Canfranc Underground Laboratory (LSC), in Spain. This paper describes the detector and associated infrastructures.

==> pool/src/hpxe_principle_of_operation_and_resolution.tex <==
\section{Principle of operation and intrinsic resolution of a  \HPXeEL\ TPC}
\label{sec.hpxe}


\begin{figure}[bhtp!]
\centering
\includegraphics[width=0.45\textwidth]{pool/imgKr/resolution_15_bar.png}
\includegraphics[width=0.45\textwidth]{pool/imgKr/resolution_7_bar.png}
\caption{\small EL Yield and resolution terms characteristic of an \HPXeEL\ as a function of the reduced electric field for an EL gap of \NewTpcELGap\ and a value of $k \sim \NewK$ (see text for details). The left panel corresponds to a pressure of \NewPressure. The right panel corresponds to a pressure of \NewSevenBarPressureRunII. } 
\label{fig.yield}
\end{figure}

As a charged particle propagates in the dense gas of a 
\HPXeEL TPC it loses energy by ionizing and exciting atoms of the medium. The excitation energy is manifested in the prompt emission of VUV (\XeWaveLength) scintillation light. The ionization electrons (ions) left behind by the particle are prevented from recombination and drifted towards the anode (cathode) by the action of a {\em drift field}. At the end of the field cage the drifting electrons enter the electroluminescent region (ELR), defined by a transparent mesh and a uniform layer of a titanium oxide compound (ITO) named gate and the anode, respectively. The thickness of the ELR as well as the voltage drop between gate and anode are chosen to provide a reasonably large amplification of the ionization signal without further ionizing the gas. An  \HPXeEL\ is, therefore, an {\em optical TPC}, where both scintillation and ionization produce a light signal. In \NEW\ (and in NEXT-100), the light is detected by two independent sensor planes located behind the anode and the cathode. The energy of the event is measured by integrating the amplified EL signal (\st) with a plane of photomultipliers (PMTs). This {\em energy plane} also records the primary scintillation light (\so) which triggers the start-of-event (\tz).  
Electroluminescent light provides tracking as well, since it is detected a few mm away from production at the anode plane via a dense array of silicon photomultipliers (SiPMs), which constitute the  \emph{tracking plane}.

The reduced electroluminescent yield (\eg, number of photons per ionization electron entering the EL region and unit of pressure), $Y/P$, of an \HPXeEL\ is experimentally found (\cite{Oliveira:2011xk}) to be:
%
\begin{equation}
Y/P = (136 \pm 1) (E/P) - (99 \pm 4) {\rm ~[photons~electron^{-1}~cm^{-1}~bar^{-1}]}
\end{equation}
%
%
where $E/P$ is the reduced field in the ELR.

One of the crucial features of an \HPXeEL\ TPC is its excellent intrinsic energy resolution, due to the small value of the Fano factor ($F$) \cite{PhysRev.72.26} in gaseous xenon and the small fluctuations of the EL yield.  Following \cite{Oliveira:2011xk} the resolution (FWHM) of an \HPXeEL\ can be written as:
%
\begin{equation}
 R_E = 2.35 \sqrt{ \frac{F}{\bar{N}_e}
 + \frac{1}{\bar{N}_e} (\frac{J}{\bar{N}_{EL}}) 
 + \frac{1.25}{\bar{N}_{ep}}}
 \label{eq.res}
\end{equation}
%
where
$\bar{N}_e$ is the number of primary ionization electrons created per event,
$J$ is the relative variance in the number of photons per ionization electron,
$\bar{N}_{EL}$ is the number of photons produced per ionization electron and
$\bar{N}_{ep}$ reflects the number of photoelectrons produced in the PMTs per event.
The factor $1.25$ takes into account both the conversion efficiency of VUV photons into photoelectrons and the fluctuations in the photoelectron multiplication gain.
Thus, these terms represent the fluctuations in
the number of primary electrons (a small number, given the low value of the Fano factor, $F=$ \XenonFanoFactor, in gaseous xenon),
the electroluminescence yield and
in the PMTs response (which in turn depends on the light collection efficiency of the detector and the distribution of the PMT's single electron pulse height),
respectively.
In pure xenon $J / \bar{N}_{EL} \ll F$, therefore, equation \ref{eq.res} can be further simplified to \cite{Oliveira:2011xk}:

%
\begin{equation}
 R_E = 2.35 \sqrt{\frac{F}{\bar{N}_e} + \frac{1.25}{\bar{N}_{ep}}}
 \label{eq.rest}
\end{equation}
%

In equation \ref{eq.rest} the Fano factor term gives the intrinsic energy resolution of xenon. 
For an energy of production of electron-ion pair of  
$w = \XenonEnergyPerElectron$ and a value of the decay energy
$\Qbb = \XenonQbb$, one finds:
	
 %
\begin{equation}
 N_E =\frac{\Qbb}{w} = \XenonElectronsAtQbb
\end{equation}
%
and thus the intrinsic xenon resolution term has a constant value:

\begin{equation}
 R_{int} = 2.35 \sqrt{\frac{F}{\bar{N}_e}} \sim \XenonIntrinsicEnergyResolution
\end{equation}

The second term, associated to the intrinsic detector resolution reads:

\begin{equation}
 \bar{N}_{ep} = k \bar{N}_e \bar{N}_{EL}
\end{equation}
%
where $k$~is the fraction of EL photons produced per \bbonu\ decay that gives rise to the production of a photoelectron. 

\Fig \ref{fig.yield} shows the EL yield and the resolution terms for an \HPXeEL\ as a function of the reduced electric field for the following operational parameters: a) a pressure of \NewPressure\ (\NewSevenBarPressureRunII) corresponding to the nominal pressure of \NEXT\ (pressure of initial operation of \NEW);  b) an EL gap of \NewTpcELGap; and c) a value of $k \sim \NewK$ (corresponding to a light collection efficiency of \NewPMTCoverage, which is the same for \NEXT\ and \NEW). Notice that, while the resolution keeps improving with increasing reduced field, the improvement above \NewReducedField\ (a value for which the resolution reaches \NewIntrinsicEnergyResolution) is very small, while the needed voltages at the gate become very large. For the initial operation of \NEW\ the reduced field is chosen to be \NewReducedFieldRunII, in order to limit the gate voltage to moderate values (\RunFourSevenThreeFourGateVoltage\ at a pressure of \NewSevenBarPressureRunII\ and \RunFourEightFourOneGateVoltage\ at a pressure of \NewNineBarPressureRunII). Under these operating conditions, the intrinsic resolution of the chamber at \Qbb\ (for point-like energy deposits) is \NewIntrinsicEnergyResolutionRunII. 


==> pool/src/runII_operation_short.tex <==
The detector started operations at LSC late in 2016. After a short engineering run (Run I) in November-December 2016, the detector was operated continuously between March and December, 2017 (Run II). 

In order to assess the overall performance of the detector and the gas system while minimizing the effect of possible leaks as well as limiting the energy of potential sparks, the operational pressure in Run II was limited to \NewSevenBarPressureRunII\ during the first part of the data taking run. The drift field was kept at \NewDriftField\  and the reduced field in the EL region at \NewReducedFieldRunII, slightly below the expected nominal value of \NewReducedField. This translates into a gate voltage of \NewGateVoltageRunII\ and a cathode voltage of \NewCathodeVoltageRunII. Under those conditions, the chamber was extremely stable, with essentially no sparks recorded over the period.

During the second part of the run the pressure was raised to  \NewNineBarPressureRunII\ and the voltages were correspondingly adjusted to keep approximately the same drift voltage and reduced field as during the first part of the run.

%Electron lifetime was low at the beginning of the data taking, possibly due to small oxygen leaks\footnote{This led to adding an exhaustive helium leak check of the full system before filling the chamber with xenon, which has been implemented for the current data run (Run II)}, but was improved, by continuous gas circulation through the getters to an acceptable value of near \NewLifetimeMaxRunII\ towards the end of the run. 
\par


==> src/Calibration.tex <==
\section{Calibration}
\label{sec:Cal}

%Sensors calibration. I don't think sensors calibration deserves a subsection here, maybe better inside the different energy/tacking plane sections, Curro!!!???


In order to get a full understanding of our detector calibration in the full energy range 30 keV to \Qbb\ is necessary. Different radioactive sources are being used in order to cover this range.
On the one hand, radioactive sources with electronic energy depositions below 100 - 150 keV produce point-like events in this high pressure detectors allowing for a very detail map response of our detector. This map response creates a matrix between the reconstructed \textit{xy} point in the EL region and the total number of photoelectron in each PMT integrating all effects that result in different light collection (eg. effects in the EL, imperfections in the light tube coating,...). For this energy range of calibration the source used was $^{83}$Rb/$^{83}$Kr$^m$ \cite{Lippincott:2009ea, LiquidXenon_KR}. This sources emmits two conversion electrons with 32.1 and 9.4 keV with a half-life of the intermediate state of 154 ns. In practise the two electrons are observed as a single event of 41.5 keV. A few $^{83}$Rb coated zeolites are placed in a branch of the gas system parallel to the main pipes. When a calibration is needed this branch opens allowing gas circulation through it. Being a gas, the krypton gets homogeneously distributed in the detector allowing for a very fine characterization of all parts of the detector.

On the other hand, calibration at higher energies is crucial in a gaseous detector as the size of the events grows with its energy and the small geometrical effects can have large impact over the energy and tracing reconstruction. In this case, several radioactive sources are being/will be used in order to provide different energy points up to \Qbb\ . These sources are: $^{22}$Na, $^{137}$Cs, $^{60}$Co and $^{228}$Th. Three calibration ports are distributed in different parts of the pressure vessel (Fig. \ref{fig:calibrationports}). In these ports the central steel region is thinner and the inner copper shield has a hole minimising the attenuation and scattering of the gammas when entering the active volume.


\begin{figure}[h!]
\centering
\includegraphics[height=8cm]{img/calibrationPorts.png}
\caption{Cut of the NEW detector where the three calibration ports are highlighted.} \label{fig:calibrationports}
\end{figure}


%Rad sources calibration.
